A Proof Of The Block Model Threshold Conjecture

We study a random graph model named the "block model" in statistics and the "planted partition model" in theoretical computer science. In its simplest form, this is a random graph with two equal-sized clusters, with a between-class edge probability of $q$ and a within-class edge probability of $p$. A striking conjecture of Decelle, Krzkala, Moore and Zdeborov\'a based on deep, non-rigorous ideas from statistical physics, gave a precise prediction for the algorithmic threshold of clustering in the sparse planted partition model. In particular, if $p = a/n$ and $q = b/n$, $s=(a-b)/2$ and $p=(a+b)/2$ then Decelle et al.\ conjectured that it is possible to efficiently cluster in a way correlated with the true partition if $s^2 > p$ and impossible if $s^2 < p$. By comparison, the best-known rigorous result is that of Coja-Oghlan, who showed that clustering is possible if $s^2 > C p \ln p$ for some sufficiently large $C$. In a previous work, we proved that indeed it is information theoretically impossible to to cluster if $s^2 < p$ and furthermore it is information theoretically impossible to even estimate the model parameters from the graph when $s^2 < p$. Here we complete the proof of the conjecture by providing an efficient algorithm for clustering in a way that is correlated with the true partition when $s^2 > p$. A different independent proof of the same result was recently obtained by Laurent Massoulie.

==> preamble.tex <==
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{amsthm}
\usepackage{amssymb}
\usepackage{MnSymbol}
%\usepackage{homework}
\usepackage{bbm}
%\usepackage{fancyhdr}
%\usepackage{algorithmic}
\usepackage{listings}
\usepackage{enumerate}
\usepackage{cite}
\usepackage{etoolbox}

\newcommand{\cc}{\subset \subset}
\newcommand{\R}{\mathbb{R}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\CP}{\mathbb{CP}}
\newcommand{\RP}{\mathbb{RP}}
\newcommand{\B}{\mathbb{B}}
\newcommand{\T}{\mathbb{T}}
\renewcommand{\O}{\mathbb{O}}
\renewcommand{\S}{\mathbb{S}}
%\renewcommand{\H}{\mathbb{H}}
\newcommand{\emp}{\mathcal{E}}
\newcommand{\proj}{\mathbb{P}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\d}{\mathrm{d}}
\newcommand{\borel}{\mathcal{R}}
\newcommand{\1}[1]{\mathbbm{1}_{\{#1\}}}
\newcommand{\tld}{\widetilde}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\nbr}{\mathcal{N}}
\newcommand{\law}{\mathcal{L}}
\newcommand{\innerp}[2]{\langle #1, #2 \rangle}
\newcommand{\inr}[2]{\langle #1, #2 \rangle}
\newcommand{\pair}[2]{\langle #1, #2 \rangle}
\newcommand{\norm}[1]{\| #1 \|}
\newcommand{\loss}{\mathcal{L}}
\newcommand{\model}{\mathcal{M}}
\newcommand{\normal}{\mathcal{N}}
\newcommand{\ind}{\perp\!\!\!\perp}
\newcommand{\pdiff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\pdiffII}[3]{\ifstrequal{#2}{#3}
{\frac{\partial^2 #1}{\partial #2^2}}
{\frac{\partial^2 #1}{\partial #2 \partial #3}}
}
\newcommand{\diffII}[3]{\ifthenelse{\equal{#2}{#3}}
{\frac{d^2 #1}{d #2^2}}
{\frac{d^2 #1}{d #2 d #3}}
}
\newcommand{\diff}[2]{\frac{d #1}{d #2}}
\newcommand{\pdiffat}[3]{\left.\frac{\partial #1}{\partial #2}\right|_{#3}}
\newcommand{\diffat}[3]{\left.\frac{d #1}{d #2}\right|_{#3}}
\newcommand{\grad}{\nabla}
\newcommand{\ostat}[2]{#1_{(\lfloor #2 \rfloor)}}
\newcommand{\nnorm}[1]{|\! | \! | #1 |\! |\! |}
\newcommand{\ac}{\prec}
\newcommand{\wh}{\widehat}
\newcommand{\wt}{\widetilde}
\newcommand{\wl}{\overline}
\renewcommand{\L}{\mathcal{L}}
\newcommand{\coeff}[1]{\langle #1 \rangle}
\newcommand{\eps}{\epsilon}
\newcommand{\lam}{\lambda}
%\newcommand{\implies}{\Rightarrow}
%\renewcommand{\Pr}{\textrm{Pr}}
\let\Pr\relax
\DeclareMathOperator{\Pr}{Pr}
\DeclareMathOperator{\nullsp}{null}
\DeclareMathOperator{\adj}{adj}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\Cov}{Cov}
\DeclareMathOperator{\Id}{Id}
\DeclareMathOperator*{\argmin}{arg\ min}
\DeclareMathOperator*{\argmax}{arg\ max}
\DeclareMathOperator{\pois}{Pois}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\interior}{Int}
\DeclareMathOperator{\Lie}{Lie}
\DeclareMathOperator{\Adj}{Adj}
\DeclareMathOperator{\Hom}{Hom}
\DeclareMathOperator{\Sym}{Sym}
\DeclareMathOperator{\Alt}{Alt}
\DeclareMathOperator{\id}{id}
\DeclareMathOperator{\range}{range}
\DeclareMathOperator{\Range}{Range}
\DeclareMathOperator{\tail}{\mathbf{tail}}
\DeclareMathOperator{\esssup}{ess\ sup}
\DeclareMathOperator{\supp}{supp}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Int}{int}
\DeclareMathOperator{\Div}{div}
\DeclareMathOperator{\tr}{tr}

\DeclareMathOperator{\bias}{BIAS}
\DeclareMathOperator{\MSE}{MSE}
\DeclareMathOperator{\MISE}{MISE}
\DeclareMathOperator{\Ber}{Bernoulli}
\DeclareMathOperator{\Binom}{Binom}
\DeclareMathOperator{\Pois}{Pois}
\DeclareMathOperator{\Hess}{Hess}

\DeclareMathOperator{\ARMA}{ARMA}
\DeclareMathOperator{\ARIMA}{ARIMA}
\DeclareMathOperator{\MA}{MA}
\DeclareMathOperator{\AR}{AR}

\DeclareMathOperator{\Inf}{Inf}
\DeclareMathOperator{\Cut}{Cut}
\DeclareMathOperator{\MaxCut}{MaxCut}
\newcommand{\Stab}{\mathbb{S}}

\newcommand{\toLp}[1]{\stackrel{L_{#1}}{\to}}
\newcommand{\toP}{\stackrel{P}{\to}}
\newcommand{\toD}{\stackrel{d}{\to}}
\newcommand{\toas}[1]{\stackrel{#1}{\to}}
\newcommand{\toAS}{\stackrel{a.s.}{\to}}
\newcommand{\toLaw}{\stackrel{\mathcal{L}}{\to}}
\newcommand{\toWeak}{\Rightarrow}
\newcommand{\eqLaw}{\stackrel{\mathcal{L}}{=}}
\newcommand{\eqD}{\stackrel{d}{=}}
\newcommand{\eqDef}{\stackrel{def}{=}}

\newcommand{\balpha}{\boldsymbol{\alpha}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\symdiff}{\Delta}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{question}[theorem]{Question}

\def \bangle{ \atopwithdelims \langle \rangle}

\newtheoremstyle{example}{\topsep}{\topsep}%
     {}%         Body font
     {}%         Indent amount (empty = no indent, \parindent = para indent)
     {\bfseries}% Thm head font
     {}%        Punctuation after thm head
     {\newline}%     Space after thm head (\newline = linebreak)
     {\thmname{#1}\thmnumber{ #2}\thmnote{ #3}}%         Thm head spec

\theoremstyle{example}
\newtheorem{example}[theorem]{Example}
%\newcommand{\Pr}{\mathbb{P}}

%\name{Joe Neeman}

